Model-Agnostic Graph Regularization for Few-Shot Learning

In many domains, relationships between categories are encoded in the knowledge graph. Recently, promising results have been achieved by incorporating knowledge graph as side information in hard classification tasks with severely limited data. However, prior models consist of highly complex architectures with many sub-components that all seem to impact performance. In this paper, we present a comprehensive empirical study on graph embedded few-shot learning. We introduce a graph regularization approach that allows a deeper understanding of the impact of incorporating graph information between labels. Our proposed regularization is widely applicable and model-agnostic, and boosts the performance of any few-shot learning model, including fine-tuning, metric-based, and optimization-based meta-learning. Our approach improves the performance of strong base learners by up to 2% on Mini-ImageNet and 6.7% on ImageNet-FS, outperforming state-of-the-art graph embedded methods. Additional analyses reveal that graph regularizing models result in a lower loss for more difficult tasks, such as those with fewer shots and less informative support examples.

==> tbl_mini_imagenet_graph.tex <==
\begin{table}[H]
\caption{Effects of different ways of implementing graph regularization. In ``Graph Init'' we use graph regularization on the classifier while training on the base classes, and using the resulting novel class embeddings to initialize novel class classifiers. We then adapt the novel classifiers using cross-entropy loss. In ``Graph Adaptation'', we add graph regularization while adapting the novel class classifiers.}
\centering
% \fontsize{9}{9}\selectfont
\begin{tabular}{p{5cm}p{3cm}p{2cm}p{2cm}}
\toprule
\bf Model & \bf Backbone & \bf 1-shot & \bf 5-shot \\
\midrule
$\text{S2M2}_R$ & WRN 28-10 & 64.93 $\pm$ 0.18 & 83.18 $\pm$ 0.11 \\
$\text{S2M2}_R$ + Graph Init & WRN 28-10 & 66.93 $\pm$ 0.65 & 83.35 $\pm$ 0.53 \\
$\text{S2M2}_R$ + Graph Init + Graph Adaptation & WRN 28-10 & 65.66 $\pm$ 0.71 & 79.87 $\pm$ 0.51 \\
\bottomrule
\end{tabular}
\end{table}

==> tbl_removing_layers.tex <==
\begin{figure}[H]
\centering
\begin{tabular}{p{5cm}p{3cm}p{3cm}}
\toprule
\bf Ablation & \textbf{Novel 1-shot} & \textbf{All 1-shot} \\
Remove last 5 layers & 57.8 & 65.19 \\
Remove last 10 layers & 54.86 & 64.23 \\
\bottomrule
\end{tabular}
\caption{Results after removing layers of the Imagenet graph. Internal nodes lower in the hierarchy are more important.}
\end{figure}

